TANDEM: Balancing Centralized and Decentralized Critics to Address the Information Gap in Complex Multi-Agent Environments

Cooperative multi-agent reinforcement learning under centralized training with decentralized execution (CTDE) shapes decentralized policies with a centralized critic that observes the global state, then removes the critic at execution. The policies are optimized to rely on information they will not have when they act, an information gap between training and execution. It widens under partial observability, observation noise, and openness, where the set of agents and tasks present changes during an episode. Existing methods transfer centralized guidance in one direction only, removing or distilling the critic once, so the policies never rehearse acting without the critic while they can still be corrected. We propose TANDEM, which keeps one centralized critic and reads it two ways at each training step: a centralized read from the global state, and a decentralized read restricted to the information each agent will have at execution. A parameter-free gate compares the two reads for each agent and trains the policy on the decentralized read where they agree, reinstating the centralized read only where the local view is misleading. A shared target pulls the decentralized read toward the centralized one. We formalize the setting as a task- and agent-open decentralized partially observable Markov decision process (TAO-Dec-POMDP) and evaluate TANDEM on three cooperative domains, each isolating one form of the information gap: discovery for partial observability, sampling for observation noise, and openness in wildfire suppression. We compare against six CTDE baselines and ablate the gate and the shared target; the supplementary material holds the full variant sweep, diagnostics, and learning curves. We measure return at execution, once the centralized critic is removed. TANDEM is the best method on eight of the nine setups and never significantly worse than any baseline.

==> figs/old_contents/3-problem.tex <==

In this section, we define the \textbf{open Dec-POMDP}, an extension of the
Dec-POMDP~\citep{oliehoek2016decpomdp} (see Section~\ref{sec:bg-decpomdp}), to
consider the conditions under which the information gap is felt (see
Sections~\ref{sec:bg-perception} and~\ref{sec:bg-openness}): openness, partial
observability, and observation noise. Under openness, both the set of agents
and the set of tasks may change during an episode, so which agents act and
which actions each of them has are properties of the current state. Under
partial observability, each agent reads that state through a local observation
rather than the state itself. Under observation noise, that observation is
further perturbed before the agent acts on it. Thus, a policy must act on the
agents and the actions that are present at the current timestep and on what its
own observation reports of them, rather than assume a fixed set of agents and
fixed action labels with permanent meaning. The Dec-POMDP represents only
partial observability, so we add two state-dependent components for openness
and define observation noise outside the tuple.

In the rest of this section, we first define the model
(Section~\ref{sec:problem-model}). We then define each condition in the model
and instantiate it in the domain where it is most pronounced: openness in
wildfire suppression~\citep{patino2025inaugural}
(Section~\ref{sec:problem-openness}), partial observability in Level-Based
Foraging~\citep{papoudakis2021benchmark} (Section~\ref{sec:problem-po}), and
observation noise in SMACv2~\citep{ellis2023smacv2}
(Section~\ref{sec:problem-noise}).

\subsection{The Open Dec-POMDP}
\label{sec:problem-model}

Consider:
\[
\mathcal{M} \;\triangleq\;
\langle \mathcal{N}, \mathcal{S}, \{\mathcal{A}_i\}, P, R, \{\Omega_i\}, O,
\gamma, \xi, \{\eta_i\} \rangle,
\]
where every component is as in Section~\ref{sec:bg-decpomdp} except the
following. $\mathcal{N}$ is the set of agents that can ever be present, rather
than a fixed set that is present throughout the episode. We add two
deterministic functions of the state. The \emph{participation function} $\xi :
\mathcal{S} \to 2^{\mathcal{N}}$ returns the active set $\mathcal{N}^t =
\xi(s^t) \subseteq \mathcal{N}$, and the \emph{availability function} $\eta_i :
\mathcal{S} \to 2^{\mathcal{A}_i}$ returns the set $\mathcal{A}_i^t =
\eta_i(s^t) \subseteq \mathcal{A}_i$ of actions available to agent $i$. We
require $\eta_i(s) \neq \emptyset$ for every $i \in \xi(s)$, so that an active
agent always has at least one action to select, which the \textsc{no-op} of our
instantiations provides.

The remaining components of $\mathcal{M}$ are defined on the active set and the
available actions at each timestep. Only active agents select actions and
receive observations. The joint action $\mathbf{a}^t$ collects the actions of
the agents in $\mathcal{N}^t$, so $P$ and $R$ are defined on $s^t$ together
with those actions, and $O$ produces one observation for each agent in
$\mathcal{N}^t$. Changes in participation and availability are induced by the
stochastic transition $P$, while $\xi$ and $\eta_i$ only read the state that
$P$ produced. This lets the model account for arbitrary change in the set of
agents and in the set of actions through the state alone, without a separate
process for either. We allow $\mathcal{N}^t = \emptyset$, in which case no
agent acts, the state still evolves under $P$, and $R$ still contributes to the
return. Setting $\xi(s) = \mathcal{N}$ and $\eta_i(s) = \mathcal{A}_i$ for all
$s \in \mathcal{S}$ recovers the Dec-POMDP of Section~\ref{sec:bg-decpomdp}.

\subsection{Openness}
\label{sec:problem-openness}

The two functions carry the two forms of openness. Agent openness is a change
in the active set $\mathcal{N}^t$ within an episode, and task openness is a
change in the available action set $\mathcal{A}_i^t$. We model task openness
through $\eta_i$ under the assumption that the actions addressing a task appear
and disappear with the task, which holds in our wildfire instantiation because
each fire carries one suppression action.

We instantiate openness using the wildfire suppression
domain~\citep{patino2025inaugural} of Section~\ref{sec:bg-openness}, a grid
where firefighter agents are stationed in fixed positions and each fire is a
task with a location and a size. Fires may ignite, spread, burn out, or be
extinguished by firefighters, changing the set of active tasks and creating
task openness. At each timestep, an agent chooses to either suppress a fire or
remain idle (\textsc{no-op}); it may also exit the environment when out of
suppressant, creating agent openness. Now, let \textsf{suppress}$(x)$ denote
the action of suppressing fire $x$.

\textbf{Task Arrival.} If a new fire $x_{\text{new}}$ ignites at time $t$, and
no existing fire is removed and no agent enters or leaves, then $s^{t+1}$
records the new fire and $\mathcal{A}_i^{t+1} = \mathcal{A}_i^t \cup
\{\textsf{suppress}(x_{\text{new}})\}$ for every agent $i \in
\mathcal{N}^{t+1}$, corresponding to $\eta_i(s^{t+1})$.

\textbf{Agent Departure.} If agent $i$ depletes its suppressant and exits at
time $t$, and no other agent enters or leaves, then $s^{t+1}$ records its
absence and $\mathcal{N}^{t+1} = \mathcal{N}^t \setminus \{i\}$, corresponding
to $\xi(s^{t+1})$. Agent $i$ selects no action and receives no observation
until a later state returns it to the active set.
%
%Frame openness, the third form of openness in Section~\ref{sec:bg-openness}, is
%outside our scope. $\mathcal{M}$ fixes each agent's frame, and a change in
%$\mathcal{A}_i^t$ reflects which tasks exist rather than what an agent is
%capable of.

\subsection{Partial Observability}
\label{sec:problem-po}

The Dec-POMDP of Section~\ref{sec:bg-decpomdp} already models partial
observability through its observation function $O$: an active agent receives
$o_i^t$ drawn from $O$ and never the global state $s^t$, and beyond its own
$\mathcal{A}_i^t$ it does not read which other agents are active or which tasks
exist.

We instantiate partial observability using Level-Based
Foraging~\citep{papoudakis2021benchmark}, a grid where each agent and each item
carries a level, and an item is collected when the levels of the agents acting
on it together meet its own. At each timestep, an agent moves, attempts to
collect an adjacent item, or remains idle (\textsc{no-op}). We use the
sight-limited \texttt{2s} configurations, in which $o_i^t$ covers the
$5\times5$ window centered on agent $i$, so agents and items outside that
window are in $s^t$ but not in $o_i^t$.

\subsection{Observation Noise}
\label{sec:problem-noise}

The Dec-POMDP of Section~\ref{sec:bg-decpomdp} does not model observation
noise, since it delivers to each agent the observation that $O$ produced.
Following the robust reinforcement learning formulation of
Section~\ref{sec:bg-perception}~\citep{zhang2020robust,he2023robust}, we write
$B_i(o_i^t) \subseteq \Omega_i$ for a perturbation set around $o_i^t$, and let
the agent act on some $\tilde{o}_i^t \in B_i(o_i^t)$ in place of $o_i^t$, where
the unperturbed case is $B_i(o_i^t) = \{o_i^t\}$. We define $B_i$ outside
$\mathcal{M}$, because it perturbs what an agent reads and leaves $s^t$,
$\mathcal{N}^t$ and $\mathcal{A}_i^t$ as the environment produced them.

We instantiate observation noise using SMACv2~\citep{ellis2023smacv2}, a team
battle in which each agent controls one unit and chooses at each timestep to
move, to attack an enemy in range, or to remain idle (\textsc{no-op}). Each
$o_i^t$ is a vector of $d_i$ continuous features such as unit health, relative
distances, and weapon cooldowns, so $\Omega_i \subseteq \mathbb{R}^{d_i}$ and a
bounded perturbation is meaningful in every coordinate. For a perturbation
budget $\delta > 0$ we take $B_i(o_i^t) = \{\tilde{o} \in \Omega_i :
\|\tilde{o} - o_i^t\|_\infty \le \delta\}$.

==> tables/captions.tex <==
% Suggested captions, one per table and figure; each states what "statistically significant" means.
% table1_results_execution
\caption{Execution return (mean over 100 unseen episodes, critic removed, one training seed) of TANDEM and the six CTDE baselines on nine setups: two with an information gap per domain and one control without it. Bold: best per setup. Superscript $k$: the number of the six baselines against which TANDEM's return is higher and the difference is statistically significant. Statistical significance: a paired two-sided Wilcoxon signed-rank test over the same 100 unseen execution episodes (unseen environment seeds 201--300, identical for every method, pairs matched by seed), $p<0.05$ after Bonferroni correction over the six baseline comparisons of a setup.}

% table2_ablate_the_gap
\caption{Execution return (mean over 100 unseen episodes) of TANDEM and the two ablations gate forced closed ($\chi\equiv0$) and no shared target; spread = max $-$ min of the three per setup. One training seed.}

% table3_shared_target_at_the_critic
\caption{Fit of the decentralized read (explained variance of $V^W$ over the last 200 training episodes) and sign-disagreement fraction between the two advantages (mean over 1000 training episodes), with and without the shared target.}

% table4_gate_against_the_gap
\caption{The gate against the information gap, full method: gap = EV(centralized read) $-$ EV(decentralized read) over the last 200 training episodes; gate mean $\bar\chi$ and sign-disagreement fraction over the 1000 episodes; episodes until the 20-episode running mean of the training return first reaches 90\% of its final rise.}

% table5_training_efficiency
\caption{Mean training return over the 1000 training episodes (area under the learning curve), TANDEM and the six CTDE baselines, one training seed.}

% appendix/tableS1_all_variants_execution
\caption{Execution return (mean over 100 unseen episodes) of every TANDEM variant, IPPO, Kickstarting and IDDQN; in brackets the difference to TANDEM (row minus TANDEM), $*$ = statistically significant. Statistical significance: a paired two-sided Wilcoxon signed-rank test over the same 100 unseen execution episodes (unseen environment seeds 201--300, identical for every method, pairs matched by seed), $p<0.05$ after Bonferroni correction over the seven comparisons of a setup.}

% fig1_results_execution
\caption{Execution return of TANDEM and the six CTDE baselines per setup (mean over 100 unseen episodes; error bars: standard error over those episodes; one training seed). The label $k/6$ over a TANDEM bar is the number of the six baselines against which TANDEM's return is higher and the difference is statistically significant. Statistical significance: a paired two-sided Wilcoxon signed-rank test over the same 100 unseen execution episodes (unseen environment seeds 201--300, identical for every method, pairs matched by seed), $p<0.05$ after Bonferroni correction over the six baseline comparisons of a setup.}

% fig2_gap_and_shared_target
\caption{Left: sign-disagreement fraction between the centralized and the decentralized advantage against the information gap (EV of the centralized read minus EV of the decentralized read, last 200 training episodes), one point per setup; marker shape = domain, hollow = control without a gap. Right: the same fraction with and without the shared target on the six gap setups (the controls are zero for both).}

% fig3_learning_curves
\caption{Training return (20-episode running mean) of TANDEM and its two ablations, gate forced closed ($\chi\equiv0$) and no shared target, with MAPPO as reference, per setup; one training seed, so no band.}

% fig4_train_vs_execution
\caption{Mean training return over episodes 901--1000 (left point) joined to the mean execution return over 100 unseen episodes (right point), per method and setup.}

% fig5_gate_dynamics
\caption{TANDEM's gate mean $\bar\chi$ and sign-disagreement fraction over training (20-episode running mean), per setup: both stay at zero on the controls without a gap.}

% fig6_training_curves_all
\caption{Training return (20-episode running mean) of TANDEM and the six CTDE baselines, one panel per setup; one training seed.}

% fig7_validation_curves_all
\caption{Validation return during training (every 40 episodes, mean over the validation episodes on the unseen validation seeds 101..; 30 episodes for discovery and sampling, 50 for wildfire), TANDEM and the six CTDE baselines, one panel per setup.}


==> tables/table1_results_execution.tex <==
\begin{tabular}{lccccccccc}
\toprule
Method & \makecell{Discovery\\3 agents, 4 targets} & \makecell{Discovery\\4 agents, 6 targets} & \makecell{Discovery\\full observation (control)} & \makecell{Sampling\\noise 0.1} & \makecell{Sampling\\noise 0.2} & \makecell{Sampling\\no noise (control)} & \makecell{Wildfire\\wf2, open} & \makecell{Wildfire\\wf3, open} & \makecell{Wildfire\\wf0, closed (control)} \\
\midrule
TANDEM & \textbf{3.70$^{6}$} & \textbf{6.91$^{6}$} & \textbf{6.29$^{5}$} & \textbf{38.87$^{5}$} & \textbf{37.79$^{6}$} & \textbf{41.16$^{6}$} & \textbf{290.1$^{5}$} & 306.6$^{5}$ & \textbf{48.00$^{6}$} \\
\midrule
MAPPO & 2.63 & 5.48 & 5.99 & 37.42 & 31.68 & 39.19 & 251.5 & \textbf{315.3} & 42.40 \\
COMA & 0.88 & 1.68 & 0.77 & 20.34 & 9.09 & 17.97 & 284.5 & 290.5 & 19.68 \\
QMIX & 1.12 & 1.93 & 1.10 & 6.81 & 4.67 & 5.27 & -60.00 & -60.00 & -23.76 \\
MADDPG & 0.96 & 2.23 & 0.99 & 5.37 & 7.37 & 13.43 & 181.8 & 202.5 & -13.44 \\
VDN & 0.81 & 1.79 & 0.84 & 17.38 & 18.83 & 6.49 & 79.24 & 41.60 & -20.32 \\
MAVEN & 1.10 & 2.07 & 0.85 & 6.79 & 5.70 & 7.05 & 40.48 & -60.00 & -9.84 \\
\bottomrule
\end{tabular}
% Execution return: mean over the 100 unseen episodes (critic removed), one training seed. Bold = best per setup. Superscript on TANDEM = number of baselines it beats significantly (paired Wilcoxon over the shared 100 episodes, Bonferroni over the baselines of that setup).
% caption: Execution return (mean over 100 unseen episodes, critic removed, one training seed) of TANDEM and the six CTDE baselines on nine setups: two with an information gap per domain and one control without it. Bold: best per setup. Superscript $k$: the number of the six baselines against which TANDEM's return is higher and the difference is statistically significant. Statistical significance: a paired two-sided Wilcoxon signed-rank test over the same 100 unseen execution episodes (unseen environment seeds 201--300, identical for every method, pairs matched by seed), $p<0.05$ after Bonferroni correction over the six baseline comparisons of a setup.


==> tables/table1_slim_results_execution.tex <==
\begin{tabular}{lccccccccc}
\toprule
Method & Disc. small & Disc. larger & Disc. control & Samp. 0.1 & Samp. 0.2 & Samp. control & WF open & WF more open & WF closed \\
\midrule
TANDEM & \textbf{3.70$^{6}$} & \textbf{6.91$^{6}$} & \textbf{6.29$^{5}$} & \textbf{38.87$^{5}$} & \textbf{37.79$^{6}$} & \textbf{41.16$^{6}$} & \textbf{290.1$^{5}$} & 306.6$^{5}$ & \textbf{48.00$^{6}$} \\
MAPPO (base) & 2.63 & 5.48 & 5.99 & 37.42 & 31.68 & 39.19 & 251.5 & \textbf{315.3} & 42.40 \\
Best competing baseline & QMIX 1.12 & MADDPG 2.23 & QMIX 1.10 & COMA 20.34 & VDN 18.83 & COMA 17.97 & COMA 284.5 & COMA 290.5 & COMA 19.68 \\
\bottomrule
\end{tabular}

